FedVal: Different good or different bad in federated learning

Federated learning (FL) systems are susceptible to attacks from malicious actors who might attempt to corrupt the training model through various poisoning attacks. FL also poses new challenges in addressing group bias, such as ensuring fair performance for different demographic groups. Traditional methods used to address such biases require centralized access to the data, which FL systems do not have. In this paper, we present a novel approach FedVal for both robustness and fairness that does not require any additional information from clients that could raise privacy concerns and consequently compromise the integrity of the FL system. To this end, we propose an innovative score function based on a server-side validation method that assesses client updates and determines the optimal aggregation balance between locally-trained models. Our research shows that this approach not only provides solid protection against poisoning attacks but can also be used to reduce group bias and subsequently promote fairness while maintaining the system's capability for differential privacy. Extensive experiments on the CIFAR-10, FEMNIST, and PUMS ACSIncome datasets in different configurations demonstrate the effectiveness of our method, resulting in state-of-the-art performances. We have proven robustness in situations where 80% of participating clients are malicious. Additionally, we have shown a significant increase in accuracy for underrepresented labels from 32% to 53%, and increase in recall rate for underrepresented features from 19% to 50%.

==> 3_method_old.tex <==
\section{FedVal}
In this Section \ref{sec:relatedwork}, we highlighted that outlier-based defenses can struggle against state-of-the-art model poisoning attacks and norm bounding mechanism may not be strong enough for defense. On the other hand, Loss Function based defenses, although computationally heavy, may provide the necessary level of validation and robustness to ensure fairness and robustness in a federated setting. Therefore, we present our innovative method \emph{FedVal} in this section. \emph{FedVal} attaches a weight based on the performance for each client model to the aggregation of their updates, which allows a more dynamic and nuanced approach to protect the global model, as opposed to traditional methods such as outlier-removal or methods that removing a set number of weights or updates.

%In order to protect the global model from bad or malicious updates and improve fairness between labels in Federated Learning systems, we propose a novel approach of using a lightweight server-side validation dataset. Our method, called FedVal, attaches a weight based on the performance of each client model to the aggregation of their updates. This allows for a more dynamic and nuanced approach to protecting the global model, as opposed to traditional methods such as outlier-removal or methods that removing a set number of weights or updates.\newline


One key advantage of score-based methods like \emph{FedVal} is that they never discard good model parameters. Other solutions that commonly remove a set number of clients' updates or norms in each round \cite{shejwalkar2021manipulating,panda2022sparsefed,blanchard2017machine,fang2020local,yin2018byzantine,li2020learning,li2019abnormal}, can fail to deal with data heterogeneity issues and cause to lose good data during the aggregation stage.
%result in problems with solving non-IID data issues and loss of good data.


While the primary goal of \emph{FedVal} is to protect the global model from malicious client updates, we have also incorporated a variable for further improvement from the average clients' model. The variable aims to decrease the potential negative effects caused by the defense mechanism to improve the fairness of FL system and model performance in the non-IID data distribution situation.
%that defenses can have on solving fairness in non-IID FL systems and even radically improve the performance of the model in the non-IID client data distribution situations.
%addresses the issue of improvements on what the average clients' models are missing. This variable aims to decrease the potential negative effects that defenses can have on solving fairness in non-IID FL systems and even radically improve the performance of the model in some non-IID client data distribution situations.


\emph{FedVal} aim to solve interplay between fairness and robustness in FL as illustrated in a example in Figure \ref{fig:example}. In this example, there are total $4$ classes in the classification task, and $4$ clients are selected in a FL communication round. $2$ of the clients has updated the model in similar directions, but they are missing one of the four classes. One of the client models is slightly worse than the first two but has information on the class that they are missing. The last client is malicious and has sent back a completely ruined model. 


Figure \ref{fig:example} highlights the advantage of \emph{FedVal} as the algorithm notices that the third client has updated the model with new information that other clients are missing and responds by aggregating that clients model by a higher factor. \emph{FedVal} also notices that there is a malicious client, and responds by not using the malicious client for the aggregation. 


On the other hand, other robust aggregators would typically favor the two most similar clients and use them for the aggregation. If a simple averaging method such as FedAvg is used, the new model would be completely deteriorated by the malicious update. But even in a situation with no malicious updates, the new information from client three is in most cases lost since the norms with the specific information for class three get under-valued compared to those of the majority client update models.

\begin{figure}[H]
\centering
\includegraphics[width=0.95\linewidth]{aggExample.png}
\caption{Theoretical example of a federated learning situation with four clients being aggregated, two majority clients with skewed data, one client with information the majority of clients are missing, and one malicious client.}
\label{fig:example}
\end{figure}

\subsection{Details}

This section will go through the details of \emph{FedVal}, illustrate how the algorithm work, and motivate the choices we made for the algorithm.

\emph{FedVal} scores each client with an adaptive function $S(\theta_c)$, which scores the client based on client performance. The function will and if the client has improved the models functionality on what the average client update for the round is missing.  Then, the central server will aggregate the model update using these score as weight of each client, as shown in the equation below:

%The aggregation of all clients into the new global model is the sum of individual norms for each client divided by what fraction of the total accumulated score each gets.

\begin{equation}\label{eq:fedval}
    \theta^{t+1}_g = \theta^{t}_g + \sum_{d}^{S_t}{\frac{S(\theta_d^{t+1})\Delta \theta^{t+1}_d}{\sum_{d}^{S_t}{S(\theta_d^{t+1})}}}
\end{equation}


The scoring function is a critical aspect of the \emph{FedVal} algorithm and plays a crucial role in achieving its objectives. Its main purpose is to extract relevant features for the model and eliminate unwanted or redundant features. This is accomplished through the use of nonlinear permutations of the loss for each label and the overall loss, which are summed together to generate an overall score for each client.


The scoring dimensions is represented as a slope determined by the mean absolute deviation (MAD) of loss across all clients in the considered dimension, and if the considered dimension is averagely falling behind for the given client updates, as illustrated in Figure \ref{fig:fedval}. 

\begin{equation}\label{eq:mad}
    MAD = \frac{\sum{|X-\mu|}}{N}
\end{equation}
where $X$ stands for ... and $\mu$ stands for ...


Another aspect regarding boosting score on dimensions that are falling behind is to not punish improvements on what the average client model is already excelling at, which can easily happen with this design if were not careful. To counteract this we limit the equation to only give additional points in dimensions that are falling behind while disregarding dimensions that are averagely ahead.\newline


This gives us the final scoring function over the label $k$, diversion from mean between clients $div$, loss function $L$, clients $d$, with hyper-parameters $s_1$, $s_2$, and $s_3$. More details regarding the algorithms can be found in Algorithm \ref{algo:fedval}.

\begin{multline}
    S(\theta_d^t) = \frac{s_1}{MAD_{avg}}*div_{avg, d} +  \\
    \sum_k (\max(1, (\frac{\barfix{\Bar{\pmb{L}}}_{labels,k}}{\pmb{\barfix{\Bar{L}}}_{avg}})^{s_3})*\frac{s_2}{MAD_{labels, k}}*div_{labels,d,k})
\end{multline}

Note that the fairness part of the algorithm $\max(1, (\frac{\barfix{\Bar{\pmb{L}}}_{labels,k}}{\pmb{\barfix{\Bar{L}}}_{avg}})^{s_3})$ can be extended to any demographic differences that might be important for the model.



\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth, trim=1cm 0cm 0cm 0cm]{Score graph.png}
\caption{Example of how the score is set for a specific label. The slope of the graph gets steeper exponentially by how much this label is behind other labels. The effect of larger or smaller deviation between client loss for the label increases or decreases the slope.}
\label{fig:fedval}
\end{figure}

As previously discussed, \emph{FedVal} has three hyper-parameters: $s_1$, $s_2$, and $s_3$, which play a crucial role in the functioning of the algorithm and each of them serves a distinct purpose. To understand their significance, let's consider their individual functions.


$s_1$ determines the relative importance of overall loss for a client compared to the loss for individual labels. If the aim is to create a model without considering fairness, and the focus is solely on minimizing potential loss, then s1 should be set to a much higher value than $s_2$. Consider that if $s1 = K * s_2$ for all classes $K$, then the impact of overall loss and individual label loss would be similar.

$s_2$, on the other hand, is the counterpart to s1 and determines the importance of individual labels in contrast to the overall loss. This hyper-parameter provides the necessary balance between individual label loss and overall loss, thus ensuring that both factors are considered in the model's training.

$s_3$, the final hyper-parameter, is where the adaptive function of the algorithm comes into play. The value of $s_3$ determines the importance of a client being good at a label where the average client updates are weaker. The effect of $s_3$ scales exponentially, meaning that the further behind a label falls, the faster it becomes more important for a client to improve their performance on that label. 

It's worth mentioning that all hyper-parameters are well correlated such that $s_1 \subset s_2 \subset s_3$ in terms of their impact on the scoring dimensions. In other words, their values are related and interdependent, ensuring that the algorithm functions optimally. 


The $s_3$ variable in our design has been made with adaptiveness in mind. This is achieved by evaluating various s3 values on the validation data set and selecting the value that results in the minimum loss. This approach can create a bias towards the distribution of the test data set, so it is important to use a test data set that is balanced and representative of the model's end goal. The set of values tested for s3 in each round are $[s3, s3+0.5, s3-0.5, s3_{high}, s3_{pre-reset}]$. The input range for s3 is set as $[3,10]$, with the starting value being the lower number and the higher number serving as $s3_{high}$. If either $s3_{high}$ or $s3_{pre-reset}$ is selected, the current value of s3 is set to $s3_{pre-reset}$ to allow a return to the optimal value found in previous rounds, in case the value was altered significantly due to an outlier round. The complete algorithm can be seen in Algorithm \ref{algo:fedval}.



\subsection{Motivation}

This design will provide a flexible defense that is prepared for any potential scenario while promoting fairness among labels and continuously striving to reduce the loss on the validation dataset during each training iteration. 


A crucial aspect to consider when discussing this type of algorithm is time complexity. It has been previously noted that exhaustively testing each client on a validation dataset can be computationally intensive \cite{li2020learning}. However, it is important to note that the actual time complexity of validating each client can be reduced by utilizing parallel processing techniques. This results in a time complexity of $O(dv)$ in parallel, where $d$ represents the dimensions of the model and $v$ represents the number of validation elements. In the experimental section of this research, we will further investigate the time complexity by examining the number of validation elements required for the defense to be robust and effective.

==> 3_method_old2.tex <==
\section{FedVal}
In Section this section we present our innovative method \emph{FedVal}. \emph{FedVal} attaches a weight based on the performance of each client model to the aggregation of their updates, which allows a more dynamic and nuanced approach to protecting the global model, as opposed to traditional methods such as outlier-removal methods or methods that remove a set number of weights or updates.

The core of \emph{FedVal} is the score function, which is used to score each client based on their performance, as determined by a server-side validation dataset. Let $S(\theta_d^t)$ be the score for client $d$ at round $t$. The main purpose of the score function is to extract relevant features for the model and eliminate unwanted or redundant features. It is accomplished via the nonlinear permutations of the loss for each label and the overall loss, which are summed together to generate a final score for each client. The score function is defined to be the mean absolute deviation (MAD) of loss across all clients in the... 

The scoring dimensions are represented as a slope determined by the mean absolute deviation (MAD) of loss across all clients in the considered dimension, and if the considered dimension is averagely falling behind for the given client updates, as illustrated in Figure \ref{fig:fedval}. 

\begin{equation}\label{eq:mad}
    MAD = \frac{\sum{|X-\mu|}}{N}
\end{equation}
where $X$ stands for ... and $\mu$ stands for ...


Another aspect regarding boosting scores on dimensions that are falling behind is to not punish improvements on what the average client model is already excelling at, which can easily happen with this design if we are not careful. To counteract this, we limit the equation to only give additional points in dimensions that are falling behind while disregarding dimensions that are averagely ahead.


This gives us the final scoring function over the label $k$, diversion from mean between clients $div$, loss function $L$, clients $d$, with hyper-parameters $s_1$, $s_2$, and $s_3$. More details regarding the algorithms can be found in Algorithm \ref{algo:fedval}.

\begin{multline}
    S(\theta_d^t) = \frac{s_1}{MAD_{avg}}*div_{avg, d} +  \\
    \sum_k (\max(1, (\frac{\barfix{\Bar{\pmb{L}}}_{labels,k}}{\pmb{\barfix{\Bar{L}}}_{avg}})^{s_3})*\frac{s_2}{MAD_{labels, k}}*div_{labels,d,k})
\end{multline}

Note that the fairness part of the algorithm $\max(1, (\frac{\barfix{\Bar{\pmb{L}}}_{labels,k}}{\pmb{\barfix{\Bar{L}}}_{avg}})^{s_3})$ can be extended to any demographic differences that might be important for the model.


\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth, trim=1cm 0cm 0cm 0cm]{Score graph.png}
\caption{Example of how the score is set for a specific label. The slope of the graph gets steeper exponentially by how much this label is behind other labels. The effect of larger or smaller deviations between client loss for the label increases or decreases the slope.}
\label{fig:fedval}
\end{figure}

Therefore, the FL training will follow the standard communication round. At the start of each communication round, a subset of clients is selected, and current global weight parameters will be broadcast to these selected clients. Then, these selected clients will perform local training .... Lastly, the weight parameters will be aggregated using the scores of each client as weight as shown in the equation below, and the complete algorithm can be seen in Algorithm \ref{algo:fedval}:

\begin{equation}\label{eq:fedval}
    \theta^{t+1}_g = \theta^{t}_g + \sum_{d}^{S_t}{\frac{S(\theta_d^{t+1})\Delta \theta^{t+1}_d}{\sum_{d}^{S_t}{S(\theta_d^{t+1})}}}
\end{equation}

As previously discussed, \emph{FedVal} has three hyper-parameters: $s_1$, $s_2$, and $s_3$, which play a crucial role in the functioning of the algorithm, and each of them serves a distinct purpose. To understand their significance, let's consider their individual functions.

$s_1$ determines the relative importance of overall loss for a client compared to the loss for individual labels. If the aim is to create a model without considering fairness, and the focus is solely on minimizing potential loss, then s1 should be set to a much higher value than $s_2$. Consider that if $s1 = K * s_2$ for all classes $K$, then the impact of overall loss and individual label loss would be similar.

$s_2$, on the other hand, is the counterpart to s1 and determines the importance of individual labels in contrast to the overall loss. This hyper-parameter provides the necessary balance between individual label loss and overall loss, thus ensuring that both factors are considered in the model's training.

$s_3$, the final hyper-parameter, is where the adaptive function of the algorithm comes into play. The value of $s_3$ determines the importance of a client being good at a label where the average client updates are weaker. The effect of $s_3$ scales exponentially, meaning that the further behind a label falls, the faster it becomes more important for a client to improve their performance on that label. 

It's worth mentioning that all hyper-parameters are well correlated such that $s_1 \subset s_2 \subset s_3$ in terms of their impact on the scoring dimensions. In other words, their values are related and interdependent, ensuring that the algorithm functions optimally. 

The $s_3$ variable in our design has been made with adaptiveness in mind. This is achieved by evaluating various s3 values on the validation data set and selecting the value that results in the minimum loss. This approach can create a bias towards the distribution of the test data set, so it is important to use a test data set that is balanced and representative of the model's end goal. The set of values tested for s3 in each round are $[s3, s3+0.5, s3-0.5, s3_{high}, s3_{pre-reset}]$. The input range for s3 is set as $[3,10]$, with the starting value being the lower number and the higher number serving as $s3_{high}$. If either $s3_{high}$ or $s3_{pre-reset}$ is selected, the current value of s3 is set to $s3_{pre-reset}$ to allow a return to the optimal value found in previous rounds, in case the value was altered significantly due to an outlier round. 

\input{3.1_algo.tex}

\subsection{Advantage of FedVal}
\emph{FedVal} is an innovative method that aims to protect the global model from malicious client attacks, while maintaining the robustness and fairness of FL training. 

One key advantage of score-based methods like \emph{FedVal} is that they never discard good model parameters. Other solutions that commonly remove a set number of clients' updates or norms in each round \cite{shejwalkar2021manipulating,panda2022sparsefed,blanchard2017machine,fang2020local,yin2018byzantine,li2020learning,li2019abnormal}, can fail to deal with data heterogeneity issues and cause the global model to lose good data during the aggregation stage.
%result in problems with solving non-IID data issues and loss of good data.

While the primary goal of \emph{FedVal} is to protect the global model from malicious client updates, we have also incorporated a variable for further improvement from the average clients' model. The variable aims to decrease the potential negative effects caused by the defense mechanism to improve the fairness of FL system and model performance in the non-IID data distribution situation.
%that defenses can have on solving fairness in non-IID FL systems and even radically improve the performance of the model in the non-IID client data distribution situations.
%addresses the issue of improvements on what the average clients' models are missing. This variable aims to decrease the potential negative effects that defenses can have on solving fairness in non-IID FL systems and even radically improve the performance of the model in some non-IID client data distribution situations.


\emph{FedVal} aims to solve the interplay between fairness and robustness in FL as illustrated in an example in Figure \ref{fig:example}. In this example, there are total of $4$ classes in the classification task, and $4$ clients are selected in an FL communication round. $2$ of the clients have updated the model in similar directions, but they are missing one of the four classes. One of the client models is slightly worse than the first two but has information on the class that they are missing. The last client is malicious and has sent back a completely ruined model.  Figure \ref{fig:example} highlights the advantage of \emph{FedVal} as the algorithm that is able to notice the extra contribution from the third client as it has updated the model with new information that other clients are missing, hence giving it higher aggregation weight. \emph{FedVal} can also identify the malicious client and give it zero weight for aggregation.

Furthermore, other robust aggregators would typically favor the two most similar clients and use them for the aggregation. If a standard averaging method such as FedAvg is used, the new model would be completely deteriorated by the malicious update. But even in a situation with no malicious updates, the new information from client $ 3$ is in most cases lost since the norms with the specific information for class $3$ get under-valued compared to those of the majority client update models.

\begin{figure}[H]
\centering
\includegraphics[width=0.95\linewidth]{aggExample.png}
\caption{Theoretical example of a federated learning situation with four clients being aggregated, two majority clients with skewed data, one client with information the majority of clients are missing, and one malicious client.}
\label{fig:example}
\end{figure}

The design of \emph{FedVal}  will provide a flexible defense that is prepared for any potential scenario while promoting fairness among labels and continuously striving to reduce the loss on the validation dataset during each training iteration, which can be shown in more detail from our comprehensive experiments in Section \ref{sec:exp}.

Time complexity is also a crucial factor when considering defenses that validate clients on server-side validation data. It has been previously noted that exhaustively testing each client on a validation dataset can be computationally intensive \cite{li2020learning}. However, it is important to note that the actual time complexity of validating each client can be reduced by utilizing parallel processing techniques, which results in a time complexity of $O(dv)$ in parallel, where $d$ represents the dimensions of the model and $v$ represents the number of validation samples. In Section \ref{sec:timeexp}, we will further investigate the time complexity by examining the number of validation samples required for \emph{FedVal} and show that \emph{FedVal} only requires a limited number of validation samples to be effective.
